Error-Control-Coding Assisted Imaging

Error-control-coding (ECC) techniques are widely used in modern digital communication systems to minimize the effect of noisy channels on the quality of received signals. Motivated by the fact that both communication and imaging can be considered as an information transfer process, in this paper we demonstrate that ECC could yield significant improvements in the image quality by reducing the effect of noise in the physical process of image acquisition. In the demonstrated approach, the object is encoded by ECC structured light fields generated by a digital-micromirror-device (DMD) while its image is obtained by decoding the received signal collected by a bucket-detector (BD). By applying a Luby Transform (LT) code as an example, our proof-of-concept experiment validates that the object image can be effectively reconstructed while errors induced by noisy reception can be significantly reduced. The demonstrated approach informs a new imaging technique: ECC assisted imaging, which can be scaled into applications such as remote sensing, spectroscopy and biomedical imaging.

==> ECC Assisted Imaging Latex 2/NP_LT_Author.tex <==
\section*{Author contributions}
X.W. conceived the original idea and designed the LT code for experiment; Z.B. designed and assembled the optical testbed; X.W. and Z.B. conducted the experiments and analyzed the data; Z.L. and W.G. supervised the work; Z.L., W.G., B.V. and S.H. conducted the discussions of the results; X.W. and B.V. wrote the manuscript and all authors reviewed the manuscript. 

==> ECC Assisted Imaging Latex 2/NP_LT_Decoding.tex <==
\section*{Decoding Process In Imaging}\label{decoding}
%After the encoding process has been defined, the next is to design the information recovery scheme, i.e. the decoding process in imaging. There are two aspects to be considered here,

The imaging decoding consists of two main operations, namely the remapping of the received signal values into GF(2) and the decoding of object information.

%The remapping of received signal values is essential to the decoding process. Without a proper remapping, the object information cannot be successfully recovered. This is because most of the ECC codes are designed to be working on finite field $\textmd{GF}^{(2)}$ which only consists of 0 and 1\citep{lin2004error,vucetic2003space}. The resulting sum, i.e. decimal formatted values output by the BD need to be remapped back to $\textmd{GF}^{(2)}$ before being sent to the image decoder.

%{\color{blue}Recall that we only keep AA from the original binary XoR in the definition of the encoding process, then our remapping strategy here is to apply modulo-2 or other equivalent operations on received encoded values.}

\begin{figure}
  \centering
  \includegraphics[width=5in]{RemappingProcess.pdf}
  \caption{\textbf{The PDF of the received signal and its remapping.} \textbf{a}, The PDF of the received signal value when $N=3$ pixels are selected in the encoding procedure. A straightforward remapping scheme is to set thresholds at middle points between possible integers and round-off the received signal value to the closest one. Then after an additional modulo-2 operation, the received signal value can be remapped to GF(2). \textbf{b}, When the noise power becomes larger, intersections (red-colored areas) between different PDF curves will be enlarged. Thus more errors caused by decision ambiguity will be introduced into the remapping process.}\label{remapping}
\end{figure}

%\begin{figure}
%\centering
%    \mbox{
%       \subfigure[]{\scalebox{0.5}{\includegraphics{Remapping.pdf}}}}
%    \mbox{
%       \subfigure[]{\scalebox{0.3}{\includegraphics{PDF_lowSigma_PS.pdf}}}
%       \subfigure[]{\scalebox{0.3}{\includegraphics{PDF_highSigma_PS.pdf}}}}
%\caption{The PDF of received signal value $y_i$ when $N=3$ pixels are selected in the $i$th encoding procedure.}
%\label{remapping}
%\end{figure}

%BD outputs a value when a single pixel is illuminated
%BD outputs different values when pixels are illuminated one by one
%The mean of those values can be expressed as $\overline{y_0}$
Assuming for pixels with value 1, the mean value of corresponding outputs from the BD is $\overline{y_0}$, ignoring propagation attenuations and only considering AWGN noise in the receiver\citep{barrett2013foundations}, the probability-density-function (PDF) for the received signal $y_i$ obtained from the $i$th imaging encoding procedure can be expressed as\citep{parzen1962estimation},
\begin{equation}\label{PDF}
  f(y_i|m\overline{y_0})=\frac{1}{\sqrt{2\pi \sigma^2}}\textmd{exp}(-\frac{(y_i-m\overline{y_0})^2}{2\sigma^2})
\end{equation} where $m=0,1,2,\ldots,M$ and $M$ is the total number of involved pixels in the $i$th encoding and $\sigma^2$ is the receiver noise variance. As the AA part of the XoR encoding operation is carried out by the BD, an intuitive remapping of the resulting sum is to find an operation that is equivalent to modulo-2. For example, when $M=3$ pixels are involved in the $i$th imaging encoding procedure, the PDF of the resulting sum $y_i$ output by the BD is as shown in Fig. \ref{remapping}a. To achieve the remapping, we can first normalize $y_i$ into $\widehat{y_i}=y_i/y_0$ and find an integer $m_i$ which is the closest to it. Under the assumption of the equal probability for each pixel value (either 0 or 1), this decision can be made by setting thresholds at middles points between possible integers (i.e. 0.5, 1.5 and 2.5). When the obtained $m_i$ is even, the corresponding value of $y_i$ on GF(2) is 0; if $m_i$ is odd, then $y_i$ corresponds to 1 on GF(2).

%Recall that XoR operation on GF(2) can be decomposed into an AA and an additional modulo-2 operation, thus given the AA has been realized by the BD, an intuitive remapping of the resulting sum is to find an operation on real field that is equivalent to modulo-2. For example, when $M=3$ pixels are involved in the $i$th imaging encoding procedure, the PDF of the resulting sum $y_i$ output by the BD is as shown in Fig.\ref{remapping}a. To achieve the remapping, we can first normalize $y_i$ into $\widehat{y_i}=y_i/y_0$ and find an integer $m_i$ which is the closest to it. Under the assumption of the equal probability for each pixel value (either 0 or 1), this decision can be made by setting thresholds at middles points between possible integers (i.e. 0.5, 1.5 and 2.5). When the obtained $m_i$ is even, the corresponding value of $y_i$ on GF(2) is 0; if $m_i$ is odd, then $y_i$ corresponds to 1 on GF(2).

%{\color{blue}For example, as shown in Fig.\ref{remapping}(a), an illumination pattern with $N=3$ selected pixels is used in the $i$th encoding procedure while the PDF of the received signal value $y_i$ is shown in Fig.\ref{remapping}(b). Thus under the assumption of the equal probability for each pixel value (either 0 or 1), an intuitive remapping scheme is to first set multiple thresholds at middle points (i.e. 0.5$p0$, 1.5$p0$ and 2.5$p0$) between different integers (i.e. 0, 1$p0$, 2$p0$ and 3$p0$) and then round-off the received $y_i$ to the closest integer $n_i$.} With a further modulo-2 operation on $n_i$, the received signal is then remapped to its corresponding value on $GF^{(2)}$.

%In communication systems, the resulting encoded products will be either 0 or 1, depending on values of information symbols that involved.
%
%{\color{blue}Similarly we also first determine which integer $n_i$ on real field $y_i$ is more closed to and calculate the probability, and then decide which value on $\textmd{GF}^{(2)}$ $y_i$ is more likely to be and also get the corresponding probability.}

However, this \emph{hard-decisions} based remapping may bring extra errors, since red-colored intersections shown in Fig. \ref{remapping}a will cause decision ambiguity. This decision ambiguity will increase with noise, as shown in Fig. \ref{remapping}b. Consequently, \emph{soft-decisions} representing the likelihood for $y_i$ are employed in our design to enable a more accurate imaging decoding. First, the log-likelihood-ratios (LLRs) for $y_i$ relative to all possible integers values is calculated as\citep{davey1998low},
\begin{equation}\label{soft_LLR}
      L(y_i)=ln\frac{P(y_i=m\overline{y_0})}{P(y_i=0)}=\frac{(2y_i-m\overline{y_0})m\overline{y_0}}{2\sigma^2}
\end{equation} The maximum LLR $L_m$ calculated by equation (\ref{soft_LLR}) will indicate which integer $m_i$ is the most likely integer estimate for $y_i$. Then the likelihood for $y_i$ in GF(2) is obtained as,
\begin{equation}\label{soft_LLR2}
      L^{GF(2)}_i=
      \begin{cases}
        + \Delta L, &\text{when $m_i$ is odd}\\
        - \Delta L, &\text{when $m_i$ is even}\\
      \end{cases}
\end{equation}and,
\begin{equation}\label{soft_LLR2}
      \Delta L=L_m-\overline{L_m}
\end{equation}where $\overline{L_m}$ is the second largest LLR value calculated by equation (\ref{soft_LLR}).

%After the received signal have been remapped to their GF(2) equivalents via LLRs, the next is to decode the object information. With an input of $L^{GF(2)}_i$, different decoding algorithms originated from communications can be directly applied.

The obtained $L^{GF(2)}_i$ values are used to decode the object information by applying decoding algorithms from communications. Here, assuming a block code such as low-density-parity-check (LDPC) code \citep{gallager1962low} or Luby Transform (LT) code \citep{luby2002lt}has been applied in the imaging encoding operation, the belief-propagation (BP) decoding algorithm\citep{mackay1995good,yue2014distributed} is given below as an example to explain the recovery procedure of the object information.

%By using circle-shaped nodes to represent different encoded signal values and square-shaped nodes to represent different pixels, the physical encoding procedures shown in Fig.\ref{EncodingProcess}b can be further represented by a bipartite graph\citep{tanner1981recursive,asratian1998bipartite} in Fig.\ref{BP_explaination_Code}. Solid lines between circles and squares describe the relationships between received signal values and illuminated pixels established by light fields generated by the DMD. Since in one encoding procedure only the information from illuminated pixels is combined into the received signal value, squares corresponding to the same illumination are connected to the same circle in the bipartite graph. However, in order to create redundancy, the same pixel will be illuminated multiple times. Thus we can also find different circles are sometimes connected to the same square.
%\begin{figure}
%  \centering
%  \includegraphics[width=5in]{BPexp.pdf}
%  \caption{\textbf{The encoding procedure represented by a bipartite graph.} Circle-shaped nodes in the graph are representing received signal values and square-shaped ones are representing pixels. {\color{blue}Numbers in squares are indicating the order of pixels while numbers in circles are representing the order of illuminations.} Solid lines are expressing relationships between pixels and received signal values introduced by light fields generated by the DMD. Orange colored nodes are directly connected to each other via orange colored solid lines. Nodes colored in blue are providing extra messages to orange ones via blue colored solid lines.}\label{BP_explaination_Code}
%\end{figure}

Taking advantage of the relationships expressed by solid lines in the bipartite graph shown in Fig. \ref{BP_explaination_Code} and using the LLRs of the received signal values obtained from remapping as \emph{a priori} information, the basic idea behind the BP algorithm is to obtain estimates of the pixel transmissivity by iteratively exchanging messages between illuminated pixel nodes and signal nodes\citep{pearl1982reverend}. First, $M_{j,i}$ representing the message passing from the $i$th signal node to the $j$th pixel node is initialized by,
\begin{equation}\label{LLR_initialization}
  M_{j,i}=L^{GF(2)}_i
\end{equation} Then in each BP iteration, $E_{j,i}$ representing the message passing from the $j$th pixel node to $i$th signal node is firstly calculated by using other indirect connected signal nodes,
\begin{equation}\label{BP_E}
  E_{j,i}=2tanh^{-1}(\prod_{i{'}\in B_j,i{'}\neq i}tanh(M_{j,i{'}}/2))
\end{equation} where $B_j$ is the set of the received signal nodes connected to the $j$th pixel node and,
\begin{equation}\label{tanh}
  2tanh^{-1}(p)=log\frac{1+p}{1-p}
\end{equation} Then $M_{j,i}$ is updated by summing up messages from all the indirect connected pixel nodes and its initial value,
\begin{equation}\label{BP_object_LLR}
    M_{j,i}=L^{GF(2)}_i+\sum_{j^{'} \in A_i,j^{'}\neq j}E_{j^{'},i}
\end{equation} where $A_i$ is the set of the illuminated pixel nodes that connected to the $i$th signal node. By iteratively repeating the calculation of $M_{j,i}$ and $E_{j,i}$, messages are generated and exchanged until the stopping criterion has been reached, i.e. either when a correct sequence is decoded or a maximum number of iterations has been reached. After the BP algorithm has been terminated, the resulting LLR of the $j$th pixel node is expressed as,
\begin{equation}\label{BP_result_LLR}
    L_j=\sum_{i\in B_j}M_{j,i}
\end{equation} and the resulting LLR of the $i$th received signal node is expressed as,
\begin{equation}\label{BP_result_LLR2}
    S_i=L_i^{GF^{(2)}}+\sum_{j\in A_i}E_{j,i}
\end{equation} Then the final decoded value $I_j$ for the $j$th pixel is determined by,
\begin{equation}\label{Final_result}
      I_j=
      \begin{cases}
        1,& \textmd{if}~L_j\geq0\\
        0,& \textmd{if}~L_j<0\\
      \end{cases}
\end{equation}

Apparently that the obtained a posteriori probability $L_j$ for the $j$th pixel value is determined not only based on the messages $L^{GF(2)}_i$ provided by directly connected received signal nodes, but also extra messages $\sum_{j^{'} \in A_i,j^{'}\neq j}E_{j^{'},i}$ obtained from other indirectly connected ones. For example, the information of the 4th pixel shown in Fig. \ref{BP_explaination_Code} is directly combined into the 1st and 2nd received signal values $y_1$ and $y_2$. Since $y_1$ also contains information from the 7th pixel, $y_2$ also includes information from 6th and 12th pixels, thus the information of the 4th pixel can be recovered with both the \emph{a priori} information provided by $y_1$ and $y_2$, as well as messages passing from other received signal values corresponding to the 6th, 7th and 12th pixels, namely $y_4$, $y_7$ and $y_8$. Consequently, even though $y_1$ and $y_2$ may be corrupted by noise, given a proper design of the ECC code, the information of the 4th pixel can still be recovered with a high probability. In other words, with the assistance from ECC codes, the object information can be protected from errors induced by noise.

When the decoding of the current received encoded sequence is finished, the decoder sends a request to the ECC encoder for sending the next encoded sequence when rateless codes are applied, while for fixed rate codes, the decoder resumes the decoding of the next received encoded sequence.




%{\color{blue} In such a manner, the object information is protected against the noise.}

%This is the reason why the information of object can be protected with the assistance from ECC code.





%The information provided by indirectly connected responses is called the extrinsic information, which can be retrieved during the BP iterative procedures presented as below,
%
%(1) Initialize LLRs for collected responses.
%
%(2) Extrinsic information from $j$th pixel to $i$th response is,
%
%
%(3) Extrinsic information from $i$th response to $j$th pixel is,
%    \begin{equation}\label{BP_object_LLR}
%      M_{j,i}=\sum_{j^{'} \in A_i,j^{'}\neq j}E_{j^{'},i+r_i}
%    \end{equation}
%
%(4) Then the total LLR for the $i$th pixel is,
%    \begin{equation}\label{BP_Final_LLR}
%      L_i=\sum_{j\in{A_i}}M_{j,i}
%    \end{equation}
%
%(5) Repeat Step (2) to Step (4) until iteration reaches the pre-defined maximum limit.
%A similar requirement can also be found in digital communication systems. After the received signal from physical channels has been down converted from the carrier-band to the base-band, a demodulator will be applied before the decoder to map the signal values back to its corresponding binary symbols.
%
%When the reception is noise-free, values in the collected response are all integers. Thus the conversion between those Real Domain integers and $GF^{(2)}$ values is intuitive: odd numbers correspond to value 1 and even numbers correspond to value 0. However, when noise is presented in the reception, those integers will be corrupted and become decimals. Then our task becomes converting Real Domain decimals to $GF^2$ values. Here, based on the strategy in handling the decimal part, we demonstrate two different types of conversion methods. The first is called a hard-decision based conversion method. Assuming the response from the pixel with value 1 is $p_0$, given the total object response collected by the BD after $N$ times measurements to be expressed as $\mathbf{R}=[r_1,r_2,\ldots,r_N]$, the procedure of this hard-decision based conversion can be presented as below,
%
%(1) Normalize $\mathbf{R}$ with $p_0$ by,
%    \begin{equation}\label{hard_normalization}
%      \bar{\mathbf{R}}=\frac{\mathbf{R}}{p_0}.
%    \end{equation}
%
%(2) Round values in $\bar{\mathbf{R}}$ to their nearest integers $\tilde{\mathbf{R}}$.
%
%(3) Divide $\tilde{\mathbf{R}}$ by 2 and get the reminders $\hat{\mathbf{R}}$.
%
%Then the response $\mathbf{R}$ collected by the BD has been converted from their original Real Domain format into $\hat{\mathbf{R}}$ in $GF^{(2)}$. It should be pointed out that in this hard-decision based conversion process, the decimal part in $\mathbf{R}$ has been directly eliminated. Thus some part of the object information could not be used in the decoding procedure afterwards.
%Alternatively, a soft-decision based process can also be used here. Instead of a direct elimination of the decimal part,


%
%
% Assuming the maximum  is expressed as $L_m$, its corresponding integer is $x_m$ and the second largest value to be $\overline{L_m}$, then
%
%
%
%
%
% in our design, probabilities are employed to describe the likelihood for the received signal value to value 1 and 0 on $GF^{(2)}$ domain. Assuming the received signal is expressed as $\mathbf{R}$ and the noise presented in the reception belongs to additive-while-gaussian-noise (AWGN) with a known power to be $\sigma^2$, the pre-processing can be presented as below,
%
%(1) Select the 1st value $r_1$ from $\mathbf{R}$.
%
%(2) Normalize $r_1$ with $p_0$ by,
%    \begin{equation}\label{hard_normalization}
%      \bar{r_1}=\frac{r_1}{p_0}.
%    \end{equation}
%
%(3) Based on 1st field pattern generated by the DMD, calculate the total number of involved pixels X.
%
%(4) Define a set of integers $\mathbf{X}=[0,1,\cdots,X]$.
%
%(5) Calculate log-likelihood-ratios (LLRs) of $\bar{r_1}$ to each integer in $\mathbf{X}$ by,
%    \begin{equation}\label{soft_LLR}
%      L(\bar{r_1}=x)=\frac{(2\bar{r_1}-x)x}{2\sigma^2}
%    \end{equation} where $x \in \mathbf{X}$.
%
%(6) Find the maximum LLR $L_m$ and its corresponding integer $x_m \in \mathbf{X}$.
%
%(7) Find the second largest LLR $\overline{L_m}$.
%
%(8) Calculate the difference by,
%    \begin{equation}\label{soft_LLR2}
%      \Delta L=L_m-\overline{L_m}
%    \end{equation}
%
%(9) Divide $x_m$ by 2 and get the reminder $\overline{x_m}$.
%
%(10) Assign positive sign to $\Delta L$ when $\overline{x_m}$ is 1. Otherwise, assign negative sign.
%
%(11) Repeat the above steps for all values in $\mathbf{R}$. 

==> ECC Assisted Imaging Latex 2/NP_LT_Discussion.tex <==
\section*{Discussion}\label{discussion}
Compared to results obtained by GI, images reconstructed by our demonstrated approach indicate a significant quality improvement under the same system settings. Although the employment of Bernoulli-distributed structured fields is physically similar to the encoding procedure in our design, it is only served for the purpose of linearly relating the GI incoherent detection fields to received signals, which is still within the framework of conventional \emph{uncoded} imaging methods. In addition, the demonstrated approach is also different from existing noise reduction techniques, since the object information is directly protected during the physical imaging process in our design rather than compensating errors in post-processing.

As seen from the experimental setup in Fig. \ref{TargetAndResult}a, the demonstrated approach possesses the same implementation complexity as a typical GI imagery. However, its reconstruction complexity may vary as the applied encoding and decoding scheme changes. For example, when a \emph{hard-decision} based non-iterative decoding method is used, the complexity of the demonstrated approach will be around $O(KlnK)$\citep{mackay2005fountain}, which is lower than the mutual-correlation based GI algorithm whose complexity is around $O(K^3)$. But when an iterative decoding method is applied, the convergence of our demonstrated approach will be determined by a variety of factors. The total number of illuminations, SNR conditions and pre-defined maximum iteration limits will all affect the termination of the BP decoding algorithm. Besides, the convergence of the BP algorithm is also related to the number of pixels involved in one encoding operation. Similarly, the termination of a GP based iterative algorithm in GI depends on the number of measurements, SNR conditions and pre-defined maximum iteration limits. Moreover, its convergence is also affected by the initial error and the condition number of the projection matrix\citep{figueiredo2007gradient}.

Besides, several aspects still need to be further investigated in our future work. In the current approach, transmissivity is selected to represent the object information and a binary-valued model is assumed. Other representations such as reflectance and refraction\citep{barrett2013foundations}, as well as quantization models such as grey-scaled ones can also be applied here. For illustration purpose, the AWGN noise from components in BD is assumed in our experiment. Thus other error sources such as Poisson-distributed photon noise and Rayleigh-distributed fading\citep{barrett2013foundations}, as well as atmosphere turbulence\citep{zhang2010correlated} need to be further investigated. In addition, ECC codes are originally designed and optimized for communication channels. In the next step, optimizations of the mathematical structure of ECC codes in the application of imaging are to be conducted.

%
%Although the proof-of-concept experiment has validated the effectiveness of our approach, several aspects still need to be investigated in our future work.
%
%(1) Quantization of object information. In our current approach, the transmissivity is selected to be the representation of object information and a binary-valued model is assumed. Since objects to be imaged are normally physical entities, other representations such as reflectance and refraction\citep{barrett2013foundations}, as well as quantization models such as multi-leveled and grey-scaled ones can also be applied here. However, it should be mentioned that when the quantization of object information is changed, the remapping and decoding schemes should also be modified accordingly. In addition, although most ECC codes are working on $\textmd{GF}^{(2)}$, some of them such as analog-fountain-codes (AFCs) are designed for real field applications\citep{shirvanimoghaddam2013near}. Thus when codes like AFCs are employed, the requirement of quantization may be further released.
%
%(2) Noise and error model. For illustration purpose, the additive-white-gaussian-noise (AWGN) model corresponding to electronic noise from components is assumed in our experiment. Thus other error sources in the reception such as Poisson-distributed photon noise and Rayleigh-distributed fading still need to be further investigated\citep{barrett2013foundations}. In addition, our current approach requires that the illumination power and duration for each pixel in one encoding procedure should be identical. Therefore, effects to the encoding process brought by propagation medium, such as propagation attenuation and atmosphere turbulence also need to be further studied.
%
%(3) Code optimization. ECC codes are originally designed and optimized for communication channels. Although our proof-of-concept experiment has demonstrated the ECC ability can be successfully enabled in the area of imaging, the mathematical structure of codes still needs to be further optimized. On the other hand, in order to achieve a low decoding complexity, the number of pixels involved in one encoding procedure should be as small as possible\citep{mackay1995good}. However, this will result in a low detection SNR since the overall illumination power on the object is determined by the number of pixels involved in each illumination. Thus a trade-off should be searched between the decoding efficiency and implementation complexity. In addition, our current approach is based on the assumption that the probability for one pixel value to be 1 and 0 is equally distributed. In order to create and add redundancy into the encoded products, the total number of encoding procedures is larger than the number of pixels at this moment. Therefore, with some additional \emph{a priori} information such as object sparsity, the total number of illuminations may be further reduced\citep{7219476}.



==> ECC Assisted Imaging Latex 2/NP_LT_Encoding.tex <==
\section*{Encoding Process In Imaging}\label{encoding}
%In general, ECC technique contains two major procedures, namely the encoding and decoding process. For adopting the ECC encoding process into the area of imaging, three aspects need to be considered here, i.e. the quantization of object information, the basic encoding operation and the generation of different encoded values. This operation is implemented by Exclusive-or (XoR) circuits.

In communication systems, the data source typically generates binary sequences, which are used as the input to the ECC encoder\citep{vucetic2003space,lin2004error}. The linear block code ECC encoding operation in a communication system starts with dividing a length $P$ message sequence into $Q$ blocks each consisting of length $K$ information symbols. As illustrated in Fig. \ref{EncodingProcess}a, each block with length $K$ is mapped into an encoded sequence of length $N$ by the ECC encoder, where $N>K$ for fixed rate codes\citep{gallager1962low} and $N=K$ for rateless codes\citep{luby2002lt}. This mapping is carried out by generating linear combinations of these $K$ binary information symbols over GF(2).

Though the target objects in imaging systems are physical entities represented by analog parameters, such as reflectance, refraction and transmissivity\citep{barrett2013foundations}, in order to simplify the application of ECC encoding we assume that the target object is represented by a binary-valued image, i.e. black and white. We choose transmissivity as an example of the physical representation of the object and divide the target object imaging plane into individual pixels whose values are defined to be either 1 or 0. Value 1 corresponds to the infinitely large transmissivity while value 0 corresponds to the infinitely small one. In such a manner, the information source in an imaging system, namely the object information, is quantized by binary-valued transmissivity and discrete pixel locations.


%selecting an information sequence of length $K$ and generating an encoded sequence of length $N$, where $N>K$, as a set of linear combinations of $K$ information symbols over GF(2). However, in imaging systems, the target objects are physical entities\citep{barrett2013foundations}. Thus to follow the analogy with communication systems and simplify the implementation of ECC for imaging systems, we assume that the target object is represented by a binary-valued image, i.e. black and white. We choose transmissivity as an example of the physical representation of the object and divide the target object imaging plane into individual pixels whose values are defined to be either 1 or 0. Value 1 corresponds to the infinitely large transmissivity while value 0 corresponds to the infinitely small one. In such a manner, the information source in an imaging system, namely the object information, is quantized by binary-valued transmissivity and discrete pixel locations.

\begin{figure}
  \centering
  \includegraphics[width=5in]{Encoding3.pdf}
  \caption{\textbf{Physical implementations of the encoding procedure.} \textbf{a}, The encoding operation in a communication system. \textbf{b}, The encoding operation in our design. \textbf{c}, The linear combination is realized by XoR operation in a communication system. \textbf{d}, The linear combination is realized by AA operations in our design and carried out by a BD. \textbf{e}, The generation of an encoded sequence in a communication system. \textbf{f}, The generation of an encoded imaging sequence in our design.}\label{EncodingProcess}
\end{figure}

In our design, the encoding operation in imaging is performed as shown in Fig. \ref{EncodingProcess}b. By following the analogy with a communication system, we divide the whole target object plane containing $P$ pixels into $Q$ squares, where each of the squares consists of $K$ pixels. Then $K$ pixels from the same square are selected to perform $N$ times imaging encoding operations and generate an encoded imaging sequence of length $N$, where $N\geq K$. In each imaging encoding operation, $M_i$ $(i=1,2,\ldots N)$ out of $K$ pixels are chosen according to a specific ECC encoding rule\citep{gallager1962low,berrou1993near,luby2002lt}. Then a DMD is used to generate a light field to simultaneously illuminate the selected $M_i$ pixels with the same intensity and duration. After the generated light field has been modulated by the object, the transmissivities of $M_i$ illuminated pixels are included in the spatial intensity distribution of the transmit-through light. While the linear combinations of information symbols in a communication encoding operation is obtained by XoR operations\citep{vucetic2003space,lin2004error} as shown in Fig. \ref{EncodingProcess}c, these operations cannot be directly realized in our scenario since the resulting transmit-through light intensity is an analog quantity. Thus in order to achieve a linear combination of the light intensity, the XoR operations are decoupled into arithmetic additions (AAs) and modulo-2 operations in our design, where AAs are carried out by a bucket-detector (BD), as illustrated in Fig. \ref{EncodingProcess}d. The resulting sum, consisting of the total intensity of the transmit-through light, is corrupted by noise, as for example additive-white-Gaussian-noise (AWGN) caused by electronic components in the BD.

As shown in Fig. \ref{EncodingProcess}e, the encoding operation in communication systems is repeated $N$ times with different combinations of involved information symbols\citep{vucetic2003space,lin2004error} in order to generate the encoded sequence of length $N$. Similarly in our design, the above imaging encoding operation is also repeated $N$ times where the selection of $M_i$ pixels is determined by the encoding rule, as illustrated in Fig. \ref{EncodingProcess}f. The obtained encoded imaging sequence of length $N$ is passed to the imaging ECC decoder, which will remap the noisy sequence into GF(2) and then perform a decoding operation similar to ECC decoding methods in communication systems.

By using circle-shaped nodes to represent different encoded signal values and square-shaped nodes to represent different pixels, this physical encoding procedure can be further represented by a bipartite graph\citep{tanner1981recursive,asratian1998bipartite} in Fig. \ref{BP_explaination_Code}. Solid lines between circles and squares describe the relationships between received signal values and illuminated pixels established by light fields generated by the DMD. Since in one encoding procedure only the information from illuminated pixels is combined into the received signal value, the squares corresponding to the same illumination are connected to the same circle in the bipartite graph. This procedure is repeated $N$ times to generate a length $N$ encoded imaging sequence.


%However, in order to create redundancy, the same pixel will be illuminated multiple times. Thus we can also find different circles are sometimes connected to the same square.
\begin{figure}
  \centering
  \includegraphics[width=5in]{BPexp.pdf}
  \caption{\textbf{The encoding procedure represented by a bipartite graph.} Circle-shaped nodes in the graph are representing received signal values and square-shaped ones are representing pixels. Numbers in squares are indicating the order of pixels while numbers in circles are representing the order of illuminations. Solid lines are expressing relationships between pixels and received signal values introduced by light fields generated by the DMD. Orange colored nodes are directly connected to each other via orange colored solid lines. Nodes colored in blue are providing extra messages to orange ones via blue colored solid lines.}\label{BP_explaination_Code}
\end{figure}





%To encode the object information, DMD selects $M$ pixels within the range of $K$ to illuminate according to a certain ECC encoding rule.
%
%The transmit-through light carries the pixels' information.
%
%To realize the linear combination operation, AA is used instead of XoR and BD is employed.
%
%$N$ encoded object information is generated by repeating the above $N$ times. Each time, the selection of pixels is different.
%
%
%
%A light beam generated from a laser source is focused on a digital-micromirror-device (DMD), which controls pixel-level reflections of the incident laser beam. By following the analogy with a communication system binary linear encoder, the DMD selects $K$ pixels on the target object imaging plane to illuminate according to a specific encoding rule\citep{gallager1962low,luby2002lt,berrou1993near}. The corresponding {\color{red}encoded imaging signal} is obtained as a linear combination of the selected $K$ pixel values. While the linear combination in communication systems is obtained by XoR operations, these operations cannot be directly performed in imaging systems, as the {\color{red}light signals} are analog. However, in our design, we decoupled XoR operations into arithmetic additions (AA) and modulo-2 operations, where the AA are carried out by a bucket detector (BD). The resulting sum, consisting of a linear combination of $K$ selected pixel values, is corrupted by additive-white-gaussian-noise (AWGN) in the BD and can be described by a Gaussian random variable with the variance of $\sigma^2$ and mean $m_0$.

%The encoding operation in imaging systems is performed as shown in the block diagram in Fig.\ref{EncodingProcess}a. A light beam generated from a laser source is focused on a digital-micromirror-device (DMD), which controls pixel-level reflections of the incident laser beam. By following the analogy with a communication system binary linear encoder, the DMD selects $K$ pixels on the target object imaging plane to illuminate according to a specific encoding rule\citep{gallager1962low,luby2002lt,berrou1993near}. The corresponding {\color{red}encoded imaging signal} is obtained as a linear combination of the selected $K$ pixel values. While the linear combination in communication systems is obtained by XoR operations, these operations cannot be directly performed in imaging systems, as the {\color{red}light signals} are analog. However, in our design, we decoupled XoR operations into arithmetic additions (AA) and modulo-2 operations, where the AA are carried out by a bucket detector (BD). The resulting sum, consisting of a linear combination of $K$ selected pixel values, is corrupted by additive-white-gaussian-noise (AWGN) in the BD and can be described by a Gaussian random variable with the variance of $\sigma^2$ and mean $m_0$.

%As shown in Fig.\ref{EncodingProcess}b, this encoding operation is repeated $N$ times to generate an imaging encoded sequence of length $N$. The imaging encoded sequence is passed to the imaging ECC decoder. As discussed in the following section, the decoder will first map the encoded noisy sequence into a GF(2) and then perform a decoding operation similar to those in communication systems ECC decoders.

%In communication systems, an encoded digital signal is typically generated by selecting an information sequence of length K and forming an encoded sequence of length N, where N>K, as a linear combination of information symbols. This operation is implemented by XoR circuits. Similarly in our design, one encoded product of object information is generated by first selecting a subset of pixels on the target imaging plane, and illuminating them simultaneously by the light field generated from the DMD. Then as shown in Fig.\ref{EncodingProcess}b, the generation of different encoded products is realized by changing the selection of pixels, i.e. the patterns of light fields generated from DMD according to the applied ECC encoding rules. The resulting encoded products of object information are collected by the BD afterwards.


%the data source typically generates binary sequences, which are used as the input to the ECC encoder. While in imaging systems, the target object is characterized by analog functions. {\color{red}For illustration purpose,} we choose transmissivity as the physical representation of the target object. To follow the analogy with communication systems and simplify the implementation of ECC for imaging systems, we assume that the target object is represented by a black and white image. We divide the target object imaging plane into individual pixels, and define pixel values to be either 1 or 0. Value 1 corresponds to the infinitely large transmissivity while value 0 corresponds to the infinitely small one. In such a manner, the object information is quantized by binary-valued transmissivity and discrete pixel locations.
%
%In communication systems the encoding operation is carried out by selecting an information sequence of length $K$ and generating an encoded sequence of length $N$, where $N>K$, as a linear combination of information symbols over the finite field GF(2). This encoding operation is implemented by Exclusive-or (XoR) circuits. In imaging systems the encoding operation is performed as shown in the block diagram in Fig\ref{EncodingProcess}. A laser illumination source generates a light beam focused on a DMD, which controls pixel level reflections of the incident laser beam. By following the analogy with a communication system binary linear encoder, the K micromirrors on the DMD are selected to illuminate the target object by using a specific encoding rule [ldpc][lt][conv code]. The corresponding encoded imaging signal is obtained by a linear combination of the selected K pixel beams modulated by the target object. While the linear combination in communication systems is obtained by XoR opeartions, these operations cannot be directly performed in imaging systems, as the light signals are analog. Consequently, in our design, we decoupled XoR operations into arithmetic additions (AA) and modulo-2 operations, where the AA are carried out by a bucket detector (BD). The resulting sum, consisting of a linear combination of K selected pixel beams, is corrupted by additive white Gaussian noise (AWGN) in the BD and can be described by a Gaussian random variable with the variance of $\sigma^2$ and mean $m_0$. This encoding operation is repeated N times, to generate an imaging encoded sequence of length N. The imaging encoded sequence is passed to the imaging ECC decoder. The decoder will first map the encoded noisy sequence into a GF(2) and then perform a decoding operation similar to those in communication systems ECC decoders. It should be mentioned that the illumination power and its duration for each selected pixel is identical.


%the application of ECC technique is normally based on a pre-condition that the information to be transmitted is discrete and digitized by binary values\citep{lin2004error,vucetic2003space}. However, in the area of imaging, most of the target objects are physical entities\citep{barrett2013foundations}. It is thus essential to select a physical representation for the object information and assign it with a proper quantization format. For illustration purpose, we choose transmissivity here as the physical representation of the object. We further divide the target imaging plane containing object into individual pixels, and assume pixel values to be either 1 or 0. Value 1 corresponds to infinitely large transmissivity while value 0 corresponds to infinitely small. In such a manner, the object information is quantized by binary-valued transmissivity and discrete pixel locations.



%Under the above quantization model, the next is to define the basic encoding operation on the object information. In communication systems, the basic encoding operation is binary exclusive-or (XoR)\citep{lin2004error,vucetic2003space}. This is because communication systems nowadays are computer or logical circuit based. However, to physically realize the binary XoR in an imaging procedure is quite challenging. Thus, a new encoding operation should be defined here with the consideration of implementation complexities. Motivated by the fact that the binary XoR can be decomposed into an arithmetic addition (AA) with an additional modulo-2 operation, we choose the AA operation which is more easily achievable as the basic encoding operation. In our design, this AA based encoding operation is physically implemented by using a digital-micromirror-device (DMD) together with a bucket-detector (BD). As shown in Fig.\ref{EncodingProcess}a, assuming there are three pixels on the target imaging plane to be encoded, the encoding operation is then realized by generating a light field using the DMD to simultaneously illuminate those pixels and collecting the encoded products by the BD. It should be mentioned that in order to guarantee information belongs to different pixels is equally included in the collected signal, the illumination power and duration for each selected pixel should be identical.

%After the basic encoding operation has been defined, now the task is to generate different encoded products of object information.

%In communication systems, an encoded digital signal is typically generated by selecting an information sequence of length K and forming an encoded sequence of length N, where N>K, as a linear combination of information symbols. This operation is implemented by XoR circuits. Similarly in our design, one encoded product of object information is generated by first selecting a subset of pixels on the target imaging plane, and illuminating them simultaneously by the light field generated from the DMD. Then as shown in Fig.\ref{EncodingProcess}b, the generation of different encoded products is realized by changing the selection of pixels, i.e. the patterns of light fields generated from DMD according to the applied ECC encoding rules. The resulting encoded products of object information are collected by the BD afterwards.

%\begin{figure}
%  \centering
%  \includegraphics[width=5in]{ImagingPlan.pdf}
%  \caption{The generation of different encoded values.}\label{GeneratingEncodeValues}
%\end{figure}

%\begin{figure}
%  \centering
%  \includegraphics[width=6in]{CodingPlan.pdf}
%  \caption{The soft-decision based BP decoding procedure. We can see from the figure that even though some part of the object response collected by the BD may be corrupted by the noise, the binary-valued pixel values can still be recovered.}\label{BP_explaination_Code}
%\end{figure}
%different encoded symbols are generated by changing the combination of information symbols involved in each binary XoR based encoding operation according to the ECC code. In our design, the generation of one encoded value is realized via the employment of the DMD-BD pair. Thus different encoded value are obtained by changing the patterns of light fields generated by the DMD according to the corresponding ECC encoding rules.


==> ECC Assisted Imaging Latex 2/NP_LT_Experiment.tex <==
\section*{A Proof-of-concept Experiment}\label{experiment}
%\begin{figure}
%  \centering
%  \includegraphics[width=5in]{TestBed2.pdf}
%  \caption{The setup of the proof-of-concept experiment.}\label{testbed}
%\end{figure}
A proof-of-concept experiment is employed to validate the effectiveness of our approach. As shown by the experiment setup in Fig. \ref{TargetAndResult}a, the testbed contains a continuous laser source, a DMD, an object, a charge-coupled-device (CCD) and a signal generator. The CCD here is used as a BD while the signal generator is used to provide synchronization between the DMD and BD. The laser source first generates a beam with a wavelength of 671nm. The beam is further adjusted by a beam expander and then uniformly projected on the DMD. By modulating the \emph{on-off} status of micromirrors on the DMD, a series of light fields are generated according to specific ECC encoding rules and projected on the object to perform encoding. With an additional collecting lens, the resulting light signals are collected by the BD afterwards and sent to the PC for decoding.

%\begin{figure}
%\centering
%    \mbox{
%       \subfigure[]{\scalebox{0.2}{\includegraphics{TestBed2.pdf}}}
%       \subfigure[]{\scalebox{0.2}{\includegraphics{GI_hollow_target.pdf}}}
%       \subfigure[]{\scalebox{0.2}{\includegraphics{2dB_LT.pdf}}}}
%%    \mbox{
%%       \subfigure[]{\scalebox{0.15}{\includegraphics{field_22.pdf}}}
%%       \subfigure[]{\scalebox{0.15}{\includegraphics{field_33.pdf}}}}
%\caption{The target object employed in the experiment and its reconstructed image.}
%\label{TargetAndResult}
%\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=5in]{SetupTarget.pdf}
  \caption{\textbf{Experiment setup and initial reconstruction result of target object.} \textbf{a}, A DMD is used to generate light fields with ECC structured patterns to encode the object information. The resulting encoded products are collected by the BD afterwards. \textbf{b}, The target object contains a \emph{GI} shaped hollow structure. \textbf{c} The reconstruction result of the object under SNR=2dB.}\label{TargetAndResult}
\end{figure}

In order to satisfy the binary-valued quantization model, we employed an object with a hollow structure in our experiment. As shown in Fig. \ref{TargetAndResult}b, it contains a \emph{GI} shaped hollow structure with a size of $2000\mu m\times 2000\mu m$. Only the light that falls into the hollow part can pass through and reach the BD. We divide the target imaging plane where object is located into $64\times 64$ pixels and assume the pixel values corresponding to the hollow part are 1. Then LT code is employed in our experiment to encode the whole $K=4096$ pixels. To perform an LT-based encoding procedure, we first choose a number $d$ from a pre-designed probability distribution $\Omega(d)$, and then randomly select $d$ pixels to illuminate. After we performed $N=8192$ times of illuminations, an image of the object is obtained by using the aforementioned BP decoding algorithm. As we can see from Fig. \ref{TargetAndResult}c, the image of object is successfully reconstructed.
\begin{figure}
  \centering
  \includegraphics[width=3.5in]{combination2.pdf}
  \caption{\textbf{Reconstruction images and MSE curves with SNR ranging from 2dB to -5dB.} \textbf{a} The reconstruction result by using the demonstrated approach. The object is stably reconstructed, indicating the object information is protected against the noise with the assistance from LT code. The reconstruction result when SNR=-5dB is presented in the insets. \textbf{b} and \textbf{c}, The reconstruction results by using conventional GI method. The object is heavily corrupted by the noise and becomes unrecognizable when SNR is lower than -3dB. The reconstruction results when SNR=-5dB are presented in the insets.}\label{MSE_LT_C_CS}
\end{figure}
As a further validation of the image quality improvement offered by the LT code, we gradually reduced the received signal-to-noise-ratio (SNR) in the reception by adding optical attenuators. First we define the SNR in our experiment as,
\begin{equation}\label{SNR_definition}
  \textmd{SNR}=10\textmd{log}_{10}\frac{P_s-P_n}{P_n}
\end{equation} where $P_s$ is the average power of the received signals and $P_n$ is the average power of background noise in the BD. Then we employ the mean-square-error (MSE) as a quantitative evaluation metric here for the reconstruction quality assessment \citep{lehmann2006theory},
\begin{equation}\label{MSEcalculation}
  \textmd{MSE}=\frac{1}{K}\sum_{j=1}^{K}(I_j-\overline{I_j})^2
\end{equation} where $K=4096$ is the total number of pixels under the current $64\times64$ resolution setting, $I_j$ is the $j$th pixel value on the obtained image and $\overline{I_j}$ is its original value. The obtained reconstruction results of the target object are presented in Fig. \ref{MSE_LT_C_CS}a. It can be seen that images of the target object are reliably reconstructed with the SNR ranging from 2dB to -5dB. Although some distortions can be observed when the SNR is down to -5dB, the major structure of the target object is still successfully reconstructed, indicating the object information is effectively protected against receiver noise by an LT code. This conclusion is also confirmed by the obtained MSE curve, which shows that the reconstruction error remains close to 0 within the evaluated SNR range.

% {\color{blue}It should also be mentioned that we actually can still get the reconstruction of object under $\textmd{SNR}=-7\textmd{dB}$ while a performance breaking down is observed around $\textmd{SNR}=-8\textmd{dB}$.}


%\begin{figure}
%\centering
%    \mbox{
%       \subfigure[]{\scalebox{0.14}{\includegraphics{2dB_LT.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{0dB_LT.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-2dB_LT.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-4dB_LT.pdf}}}}
%    \mbox{
%       \subfigure[]{\scalebox{0.14}{\includegraphics{2dB_CS.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{0dB_CS.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-2dB_CS.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-4dB_CS.pdf}}}}
%    \mbox{
%       \subfigure[]{\scalebox{0.14}{\includegraphics{2dB_C.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{0dB_C.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-2dB_C.pdf}}}
%       \subfigure[]{\scalebox{0.14}{\includegraphics{-4dB_C.pdf}}}}
%\caption{Reconstruction results of the target object with a SNR range from 2dB to -4dB.}
%\label{SNRandResults}
%\end{figure}


%\begin{figure}
%\centering
%    \mbox{
%       \subfigure[]{\scalebox{0.3}{\includegraphics{MSE_Result_LT.pdf}}}
%       \subfigure[]{\scalebox{0.3}{\includegraphics{MSE_Result_CS.pdf}}}
%       \subfigure[]{\scalebox{0.3}{\includegraphics{MSE_Result_C.pdf}}}}
%\caption{Reconstruction MSE with a SNR range from 2dB to -5dB}\label{MSE_LT_C_CS}
%\end{figure}


As a comparison, with the same system setup, SNR range and the total number of illuminations, GI is chosen here as a representative of a conventional \emph{uncoded} imaging approach. 8192 light fields with Bernoulli-distributed patterns \citep{watts2014terahertz} are generated by the DMD and used to illuminate the object. Then the received signal collected by the BD is processed with mutual-correlation \citep{zhang2009improving} and gradient-projection (GP) \citep{zhao2012ghost,gong2016three} based algorithms respectively to reconstruct the image. As we can see from Fig. \ref{MSE_LT_C_CS}b and c, images of the target object can also be recovered by using conventional GI schemes. However, the obtained images from both of the reconstruction methods contain significant distortions. When the SNR condition is down to -5dB, the target object has been completely corrupted by noise. A similar conclusion can also be drawn by the obtained MSE curves. Results from both of the two reconstruction algorithms possess a significantly larger initial MSE, compared to our demonstrated approach at $\textmd{SNR}=2\textmd{dB}$. As the SNR worsens, their MSE curves keep increase dramatically, indicating that the object information is heavily corrupted by the receiver noise.

%\begin{figure}
%  \centering
%  \includegraphics[width=5in]{MSE_LT_C_CS.pdf}
%  \caption{MSE under SNR.}\label{MSE_LT_C_CS}
%\end{figure}


%\begin{figure}
%  \centering
%  \includegraphics[width=6in]{Combination.pdf}
%  \caption{Benchmarking MSE with a SNR range from 2dB to -5dB}\label{MSE_LT_C_CS}
%\end{figure}

%By introducing mean-square-error (MSE) as a quantitative evaluation tool, a similar conclusion can also be observed.
%
%As shown in Fig.\ref{MSE_LT_C_CS}, MSE curves corresponding to the \emph{uncoded} GI scheme keep increasing significantly as the worsening of SNR conditions, indicating obtained images suffer greatly from the noise. However, within the same SNR range, the MSE curve belongs to the \emph{encoded} approach remains closely to 0, indicating the error-correction ability from LT code is enabled in our experiment and the object information is effectively protected from the reception noise.



%In the experiment, we discrete the target imaging plane into 64-by-64 pixels and assume the transmissivity at each pixel is either 1 or 0. We applied Luby Transform (LT) code which is a type of linear block codes to encode the object information here. The encoding process by using the LT code is shown as below,
%
%(1) Select a number $d$ called \emph{degree} from a purposely design \emph{degree distribution} $\Omega$.
%
%(2) Randomly select a total number of $d$ pixels on the target imaging plane.
%
%(3) Illuminate the selected $d$ pixels with equal power and time using the DMD.
%
%(4) Collect the passing-through light signal by the bucket detector.
%
%(5) Repeat the above steps until reaches the pre-determined measurement numbers. 

==> ECC Assisted Imaging Latex 2/NP_LT_Introduction.tex <==
Error-control-coding (ECC) technique has its origin in the pioneering work of Shannon's published in 1948. In his well-known paper \emph{A Mathematical Theory of Communication}, Shannon proved that by properly encoding the information, one can achieve any arbitrarily low error probability, as long as the data transfer rate does not exceed the channel capacity\citep{shannon2001mathematical}. Then in the following decades, a variety of ECC codes are invented to combat errors caused by noisy channels, providing efficient and reliable digital data transmission in commercial, governmental and military spheres\citep{hamming1950error,reed1960polynomial,bose1960class,gallager1962low,berrou1993near,luby2002lt,arikan2009channel,shirvanimoghaddam2013near}. Though there are many different classes of ECC, their underlying principle is the same, i.e. adding structured redundancy at the transmitter. By following deliberately designed encoding rules, redundancy is created and added into the transmitted encoded symbols. Thus even if some of the received symbols are corrupted by noise, the decoder can use the redundancy information to recover the original message with a high probability.

%By introducing purposely designed redundant symbols, additional information is provided to the decoder.} Thus even some of the received symbols are corrupted by the noise, the original information can still be recovered with a low error rate.
\begin{figure}
  \centering
  \includegraphics[width=5in]{CommImgDiagram.pdf}
  \caption{\textbf{A block diagram of a digital communication systems and an imaging systems.} Both of them contains an information source, an information transfer channel and an information destination. In communication systems information is encoded by ECC before transmission while there is no similar procedure in imaging systems.}\label{ImagingandCommunications}
\end{figure}

Imaging is a physical procedure which acquires the representation or reproduction of an object such as its shape, location, structure, etc. Radiations and fields such as electromagnetic waves, particles and quasistatic fields can be used to form an image\citep{barrett2013foundations}. However, no matter what physical means an imaging system applies, it is an information transfer process which can be represented by the same basic model as a communication system. As shown in Fig. \ref{ImagingandCommunications}, communication and imaging systems both contain an information source (data source in a communication system or target object in an imaging system), an information transfer channel (communication channel in a communication system or physical propagation in an imaging system) and an information destination (data sink in a communication system or obtained image in an imaging system). One of the major differences between them lies in the information processing before transmission. In communication systems, information is encoded by an ECC and transmitted over the channel. When errors occur during the information transfer process, communication systems can achieve a high reliability with the assistance from ECC codes. On the other hand, the object information can also be corrupted by noise presented in an imaging system. However, in its current framework, there is no similar procedure so far. Thus by following the analogy with communication systems, we posed a logical question: Could ECC, developed for communication systems, be applied to imaging systems to protect object information against noise and achieve a more reliable imaging performance?

In this article, we provide an initial affirmative answer to this question. Under the assumption that the object information is represented by binary-valued transmissivity, a digital-micromirror-device (DMD) is used to encode the object by light fields generated according to ECC encoding rules. Then the transmit-through lights are collected by a bucket-detector (BD) and passed to the decoder. After converting analog BD outputs to the Galois field GF(2) where most ECC codes are designed to work, the object information is recovered by applying ECC decoding algorithms designed for communication systems. Our proof-of-concept experiment validates that the object information can be effectively protected against errors induced by reception noise. Under the same system settings, the superiority of the demonstrated approach is further confirmed by benchmarking with ghost imaging (GI)\citep{pittman1995optical,gatti2004ghost,cheng2004incoherent,jiying2010high}, which is chosen to represent conventional \emph{uncoded} imaging schemes.
%{\color{red}Add possible applications here...}

%{\color{red}It should be mentioned that although the application of random structured fields in the framework of GI can be recognized as a kind of pre-processing of object information, it is only served for the purpose of establishing linear relationships between the incoherent detection fields and received signals.} In addition, the demonstrated approach is also different from existing noise reduction methods[cites], since the object information is directly protected during the physical imaging process rather than compensating errors in the post-processing {\color{blue} afterwards.}



%The demonstrated approach further extends the application of Shannon's Information Theory. It also informs a new type of imaging technique, ECC assisted imaging.

%It should be mentioned that unlike conventional ECC in communication systems, the ECC here is implemented directly at the physical level of imaging.

%The organization of the remaining of this paper is as follows. In Section \ref{encoding}, the encoding process in imaging is firstly explained, then followed by the decoding process in Section \ref{decoding}. In Section \ref{experiment} our proof-of-concept experiment is introduced to present the effectiveness of the approach, then some aspects to be further investigated is listed in Section \ref{discussion}. At last, some concluding remarks are drawn in Section \ref{conclusion}.



==> ECC Assisted Imaging Latex 2/NP_LT_Methods.tex <==
\section*{Methods}
\noindent\textbf{Experimental details.} In the present proof-of-concept experiment, the source was a 671nm semi-conductor continuous laser source. A beam expander was applied to uniform the laser beam. A Texas Instruments V-7001 DMD with $1024\times768$ micromirrors in total was used in the experiment, but only $256 \times 256$ located at the center were employed to generate light fields. The size of each micromirror was $13.6\mu m\times 13.6\mu m$. Thus the overall size of generated light fields was $3481\mu m\times3481\mu m$. The generated light fields were projected on the hollow structured object by using a 1:1 imaging lens. Then the transmit-through lights were collected by an AVT Stingray F-504C CCD with the assistance from a collecting lens. For synchronization between the DMD and CCD, a Tektronix AFG3252C Arbitrary Function Generator was used to generate a square wave with a frequency of 20MHz. For the control of SNR conditions, we used 25mm Absorptive ND Filter Kit from Thorlabs.

\noindent\textbf{Distribution $\Omega(d)$.} The distribution $\Omega(d)$ that employed in the encoding procedure in our proof-of-concept experiment is defined as follows,\\
(1) The range of $d$ is from 1 to 10;\\
(2) The probability of $d=1$ and $d=2$ is $30\%$ respectively;\\
(3) The probability for each of the rest values is $5\%$.



